Manipulation of Granular Materials by Learning Particle Interactions

Manipulation of granular materials such as sand or rice remains an unsolved problem due to challenges such as the difficulty of defining their configuration or modeling the materials and their particles interactions. Current approaches tend to simplify the material dynamics and omit the interactions between the particles. In this paper, we propose to use a graph-based representation to model the interaction dynamics of the material and rigid bodies manipulating it. This allows the planning of manipulation trajectories to reach a desired configuration of the material. We use a graph neural network (GNN) to model the particle interactions via message-passing. To plan manipulation trajectories, we propose to minimise the Wasserstein distance between a predicted distribution of granular particles and their desired configuration. We demonstrate that the proposed method is able to pour granular materials into the desired configuration both in simulated and real scenarios.

==> gnn_model.tex <==
\subsection{Graph-based representation}
\label{sec:graph_represent}

Our method makes use of a graph representation where each particle $\mathbf{p}_i$ is represented by a node in a graph $G$. The nodes are connected via edges if the particles they represent interact with each other. We assume the interaction depends on whether particles are in contact, where contact exists if their distance is lower than a threshold $R$. 

% Let's see how the end of the intro of the method flows with this. We might need a bit of intro here, maybe not
We define a graph as $G=(V,E)$, where $\mathbf{v}_i \in V$ is a node attribute vector and $\mathbf{e}_{ij} \in E$ represents an edge attribute vector, where $i$ is the index of the sender node and $j$ is the index of the receiver node.
Here, we consider that $V \in \mathbb{R}^{N \times D}$ and $E \in \mathbb{R}^{M \times F}$, where $N$ and $M$ are the number of nodes and edges, and $D$ and $F$ are the node and edge attribute dimensions, respectively.
% is the dimension of a node attribute vector, and that , where $M$ the number of edges and $F$ is the dimension of an edge attribute vector.
We define the node attribute vector as $\mathbf{v}_i = [ \mathbf{\dot{x}}_{t-5},  \cdots, \mathbf{\dot{x}}_{t-1}, \mathbf{b}_t, m, \mathbf{c}_t ]$, where $\mathbf{\dot{x}}_{t-5},  \cdots, \mathbf{\dot{x}}_{t-1}$ are the five previous velocities of the particle, $\mathbf{b}_t$ represents the relative distance to the container boundaries, $m$ denotes whether the particle is a rigid body particle or a granular material particle, and $\mathbf{c}_t$ represents the control inputs applied to the particle. The control input is defined as the current velocity of the particle $\mathbf{\dot{x}_{t}}$ for rigid-body particles, and a zero vector for granular material particles. The edge attribute vector is $ \mathbf{e}_{ij} = [ \mathbf{s}_{ij}, d_{ij}] $, where $\mathbf{s}_{ij}$ represents the relative displacement between the particles $\mathbf{s}_{ij}=\mathbf{p}_i - \mathbf{p}_j$, and $d_{ij}$ represents their relative distance.

% GNNs are oftentimes used to learn a new node representation (i.a. ?, ?, ?) but some models and frameworks also allow learning of edge representation (e.g. ?) or updating the global attributes. [TODO: Mention graph classification, graph formation as another type of GNN ?]

% GNN was proposed in \cite{Scarselli2009_graph_neural_networks_model}. Their model learns node attribute vectors $v_i$ and a node output vectors $o_i$ using two learnable functions: local transition function and local output function. Local transition function takes information of edges incident to a node and nodes adjacent to it and outputs node attribute vector $v_i$. Node attribute vectors are updated iteratively using the same function until convergence. Then the node output function computes the node output $o_i$ from the final node attribute vector and static node features. Both learnable functions may be represented by other neural network structures such as feedforward neural networks. Later GNN-based models designed for physics modeling do not work exactly as this original GNN model does, however, the idea of of node attributes being updated using the information about the surrounding nodes and edges in the graph remains.

% To allow functions to process different number of nodes and edges in different graphs many GNN models and frameworks use aggregation functions such as sums and means to combine several vectors into one. That way the number of inputs to a function will remain the same regardless of how many nodes and edges are considered. Aggregation functions also often need to give permutation invariance to the attribute vectors. That is, the order in which different node or edge attribute vectors are given to the function makes no difference. [Needs references?]

% Our architecture is based on Graph Networks-based Simulators \cite{Sanchez-Gonzalez2020_learning_to_simulate} (GNS) framework. GNS uses in its architecture multilayer perceptrons (MLP) and Graph network \cite{Battaglia2018_relational} (GN) blocks. GN blocks are basic building blocks of GN framework which allows learning of node, edge and global attributes. GN blocks are built to take a whole graph as an input and to output another updated graph. This allows chaining several GN blocks together by passing output of one GN block as an input to the next. GN blocks consist of three functions for updating attributes, $\phi^e$ for edge attributes, $\phi^v$ for node attributes and $\phi^u$ for global attributes, and three aggregation functions $\rho^{e \rightarrow v}$, $\rho^{e \rightarrow u}$ and $\rho^{v \rightarrow u}$ for combining attribute vectors into one and to be used by update functions.
%\begin{align*}
%  e_k' &= \phi^e(e_k, v_{s_k}, v_{r_k}, u)        & \overline{e}_i' &= \rho^{e \rightarrow v}(E_i') \\
%  v_i' &= \phi^v(\overline{e}_i', v_i, u)         & \overline{e}'   &= \rho^{e \rightarrow u}(E')   \\
%  u'   &= \phi^u(\overline{e}', \overline{v}', u) & \overline{v}'   &= \rho^{v \rightarrow u}(V')
%\end{align*}
%where $E_i'=\{ (s_k, r_k, e_k') \}_{r_k=i, k=1...|E|}$ represents the updated edges whose receiver node has index $i$, $E' = \{  (s_k, r_k, e_k') \}_{k=1...|E|}$ represents all updated edges, and $V' = \{ v_i' \}_{i=1...|V|}$ represents all updated nodes.
\subsection{Graph Neural Network model}
\label{sec:gnn_model}

We learn the dynamics of the granular material particles and their interaction with the rigid-body using a GNN model.
The GNN model is used to predict the accelerations of the granular material particles and their trajectories knowing their initial positions as well as the true position of the rigid-body particles.
Our network architecture is based on the  GNS framework \cite{Sanchez-Gonzalez2020_learning_to_simulate}.
The model is divided into three sequential parts: (a) an encoder $\mathbf{f}: G_{i} \mapsto G_{l}$, (b) a processor $\mathbf{g}: G_{l} \mapsto G_{K}$, and (c) a decoder $\mathbf{h}: G_{K} \mapsto A$. The encoder maps the input graph $G_{i}$ into a latent graph $G_{l}$. The processor propagates the information through $K$ latent graphs, outputting the final latent graph $G_{K}$. Finally, the decoder produces as output the acceleration of each particle represented by a node using the node attributes of the final latent graph $G_{K}$.

\paragraph{Encoder} The encoder takes an input graph $G_{i} = (V_{i}, E_{i}) $ and uses two functions $\varphi_v$ and $\varphi_e$ to encode the node attributes $V_{i} \in \R^{N \times D_{i}}$ and edge attributes $E_{i} \in \mathbb{R}^{M \times F_{i}}$ to produce a latent graph $G_{l} =  (V_{l}, E_{l})$ where $V_{l} \in \R^{N \times D_{l}}$ and $E_{l} \in \mathbb{R}^{M \times F_{l}}$ as
\begin{equation}
    \begin{aligned}
        V_{l} &= \varphi_v(V_{i}), \\
        E_{l} &= \varphi_e(E_{i}),
    \end{aligned}
\end{equation}
where $\varphi_v$ and $\varphi_e$ are multi-layer perceptrons (MLPs). 

\paragraph{Processor} The processor consists of $K$ interaction networks (IN) \cite{Battaglia2016_interaction} such that the output attributes of one network is summed to its input attributes to produce a new latent graph. The new latent graph given as input to the next network to propagate information through the graph. The output of the processor is the final latent graph $G_{K}$. Each IN is defined as
\begin{equation}
    \begin{aligned}
        \mathbf{e}'_{ij} &= \phi_e(\mathbf{e}_{ij}, \mathbf{v}_{i}, \mathbf{v}_{j}),   &  \mathbf{\overline{e}}'_{j} = \sum_{ \mathbf{e}_{ij} \in E_{j} } \mathbf{e}_{ij}, \\
        \mathbf{v}'_{i} &= \phi_v(\mathbf{v}_i, \mathbf{\overline{e}}'_{i}), & 
    \end{aligned}
\end{equation}
where $E_j = \{ \mathbf{e}_{ij} \mid i = 1,\cdots,N \}$ is the set of edges whose receiver node is node with index $j$. Functions $\phi_e$ and $\phi_v$ are MLPs such that each IN has the same architecture but different weights. 

\paragraph{Decoder} The decoder produces the output for each node using the graph produced by the final IN of the processor by
\begin{equation}
    \mathbf{\ddot{x}}_i = \varphi_a(\mathbf{v}_i)
\end{equation}
where $\mathbf{\ddot{x}}_i \in A$ is the acceleration of the particle and $\varphi_a$ is a MLP.

In order to predict the trajectory using the predicted accelerations, we use a semi-implicit Euler integration to compute the next state based on the predicted accelerations: 
% It is used as a surrogate model in order to manipulate granular materials. Current velocity $\mathbf{\dot{x}}_{i,t}$ and next position of particle $\mathbf{x}_{i,t+1}$ is computed using the current position of particle $\mathbf{x}_{i,t}$, the previous velocity of particle $\mathbf{\dot{x}}_{i,t-1}$ and predicted acceleration $\mathbf{\ddot{x}}_{i}$ as
\begin{equation}
    \begin{aligned}
        \mathbf{\dot{x}}_{i,t} &= \mathbf{\dot{x}}_{i,t-1} + \Delta t \, \mathbf{\ddot{x}}_{i,t-1}, \\
        \mathbf{x}_{i,t} &= \mathbf{x}_{i,t-1} + \Delta t \, \mathbf{\dot{x}}_{i,t}.
    \end{aligned}
\end{equation}


% I am keeping the version below as it is for now as I'm using it as reference on how to do this - Neea

% Our GNN model is based on the Graph Networks-based Simulator (GNS) framework \cite{Battaglia2018_relational}. The model we use is composed by three blocks: (1) an encoder $\mathbf{f}: G_i \mapsto G_l$ mapping the input $G_i$ to a latent graph $G_l$, (2) a processor $\mathbf{g}: G_l \mapsto G_{l+K}$ that propagates the information through $K$ latent graphs, (3) and a decoder $\mathbf{h}: G_{l+K} \mapsto X$ that maps the propagated latent graph to the predicted acceleration of the nodes $\mathbf{\ddot{x}} \in X$.

% \paragraph{Encoder} the output produces a latent graph $G_l=(V_l, E_l)$ by
% \begin{equation}
%    \begin{aligned}
%        V_l &= \varphi^v(G_i),\\
%         E_l &= \varphi^e(G_i),
%     \end{aligned}
% \end{equation}
% where $\varphi^v$ and $\varphi^e$ are multi-layer perceptron (MLP) networks.

% \paragraph{Processor} the information is propagated by using $K$ interaction networks (INs) [cite Battaglia INs]. Each IN module is computed following:
% \begin{equation}
%     \begin{aligned}
%         \mathbf{e}'_{l+1} &= \varphi^e(\mathbf{e}_l, \mathbf{v}_{l,s_l}, \mathbf{v}_{l,r_l}), 
%         & \mathbf{\overline{e}}'_{l+1} = \sum_{r_{l+1}} \mathbf{e}_{l+1}
%     \end{aligned}
% \end{equation}




==> granular_manip.tex <==
% Present manipulation objective
Our objective is to control the rigid-body particles $P_r$ by performing a trajectory $\mathcal{T}$ that leads the granular particles to the desired goal position $P_{g,G}$. 
We consider a planning horizon $H$, where the granular particles start from a initial position $P_{g,0}$ in which they are located inside the rigid-body.
% How is the trajectory optimised?
% The trajectory of the granular particles is only controllable through the rigid-body particles. 
The rigid-body can be controlled through two set of actions, rotation and translation $\mathbf{u}_t=(\mathbf{R}_t, \Delta\mathbf{x}_t)$.
% Therefore, we optimise the trajectory of the particles $P_r$ so that we minimise the distance to the desired configuration. 
The optimal trajectory is defined by the set of actions $\mathcal{T}^*=(\mathbf{u}_0, \dots, \mathbf{u}_H)$ which minimises the distance between the end position of the particles and the desired goal position:
\begin{equation}
    \mathbf{u}_0, \dots, \mathbf{u}_H = \min d(P_{g,G},P_{g,H}).
\end{equation}
% How is the distance\loss measured
% Sinkhorn divergence paper https://arxiv.org/pdf/1910.12958.pdf
% Interpolating OT and MMD using Sinkhorn divergences (geomloss paper): https://arxiv.org/pdf/1810.08278.pdf
One option to measure the error between the desired and position of the particles would be the root mean squared error (RMSE).
However, this  would complicate the trajectory optimisation problem by requiring each particle to be in a specific position. 
Instead, we decide to measure the error between the underlying particles distribution.
% Highlight optimisation problem on mapping 1-to-1
We consider the granular particles an experimental distribution that needs to be transported from $P_{g,G}$ to $P_{g,H}$.
Thus, we formulate the trajectory optimisation as a discrete optimal transport (OT) problem, where we want to minimise the quadratic Wasserstein distance 
\begin{equation}
    W_2(P_{g,G}, P_{g,H}) = \left(
    \sum_{i=0}^M \lVert X_{i,G} - X_{i,H} \rVert^2
    \right)^{1/2},
\end{equation}
where $X_{i,G} \in P_{g,G}$ and $X_{i,H} \in P_{g,H}$ are the samples of each empirical distribution.
% Mention here problem with Wasserstein distance and experimental distribution, unbalanced OT
One of the issues when computing the Wasserstein distance is the computational cost.
Therefore, we decide to take on the approach presented by \cite{feydy_2019_otsinkhorn} which scales OT to large datasets, and use the Sinkhorn loss $S_\varepsilon(P_{g,G},, P_{g,H})$ to reduce the computational cost.
% and use the Sinkhorn loss $S_\varepsilon(\pmb{\alpha}, P_{g,G}, \pmb{\beta}, P_{g,H})$, where $\pmb{\alpha} \in \R^M_+$ and $\pmb{\beta} \in \R^M_+$ are non-negative vectors that sum up to 1.


% Now move onto how we optimise the trajectory CMA-ES
In order to solve the trajectory optimisation problem using the Sinkhorn loss, we adopt a population-based black-box optimizer, the Covariance Matrix Adaptation Evolution Strategy (CMA-ES) \cite{hansen_2001_cmaes}.
In addition to minimising the distance between the experimental distributions, we also want to find a smooth trajectory to avoid abrupt changes of the rigid-body. Therefore, we include two terms that penalise the velocity and acceleration of the rigid-body.
We additionally incorporate two constraints into the pouring task: 1) the material is not poured outside the container, and 2) the rigid-body finishes with the same starting configuration. 
Therefore, we add a binary penalty term $l_b$ that is positive when the granular material is outside of the container boundaries, and a loss term for the end rotation $\theta_T$ of the rigid-body.
Our cost function is thus formulated as

\begin{equation}
\label{eqn:cost_function}
\begin{aligned}
    c(P_{g,G}, P_{g,H}, \mathcal{T}) &=
    \alpha \, S_\varepsilon( P_{g,G}, P_{g,H})
    + \beta \sum_{t=1}^H \lVert \mathbf{u}_t - \mathbf{u}_{t-1} \rVert^2 \\
    &+ \gamma \sum_{t=1}^H \lVert \mathbf{u}_t - 2\mathbf{u}_{t-1} + \mathbf{u}_{t-2} \rVert^2 \\
    +& \rho \, l_b + \omega \lVert \theta_0 - \theta_T \rVert
\end{aligned}
\end{equation}
where $\alpha$, $\beta$, $\gamma$, $\rho$ and $\omega$ are regularisation constants.

The optimal trajectory is found following the Algorithm~\ref{alg:cma-es}. On the first iteration, we take as input an initial trajectory $\mathcal{T}$ with random actions. Then, we create the graph as explained in Section~\ref{sec:graph_represent}. Here, we compute the control inputs $\mathbf{c}_t$ as the difference between $P_{r,t}$ and $P_{r,t-1}$ after applying the actions $\mathbf{u}^*_t$. On line 5 we compute the next position of the granular particles $P_{g,t+1}$ using the semi-implicit Euler formulation.
% The position of the rigid-body particles $P_{r,t+1}$ is not updated using the GNN model.
Once the rollout has finished, the cost $c(\cdot)$ is computed and the CMA-ES performs another iteration until reaching the threshold $\varepsilon$.

\begin{algorithm}
\caption{Trajectory optimisation}\label{alg:cma-es}
\begin{algorithmic}[1]
% \Require $a$
\Require $P_0$, $P_{g,G}$, $\mathcal{T}$, $\varepsilon$
\Ensure $\mathcal{T}^*$
\While{$d \leq \varepsilon$}
    \For{$t=0 \rightarrow H$}
        \State $\mathbf{u}^*_t \gets \mathcal{T}_t$ 
        \State $G_{i, t} \gets$create\_graph$(P_t, \mathbf{u}^*_t)$  \Comment{See Section~\ref{sec:graph_represent}}
        \State $P_{t+1} \gets$GNN$(G_{i, t})$
    \EndFor
    \State $\mathcal{T} = \min c(P_{g,G}, P_{g,H}, \mathcal{T})$  \Comment{Using CMA-ES}
\EndWhile
\State $\mathcal{T}^* \gets \mathcal{T}$
\end{algorithmic}
\end{algorithm}


% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{img/optimal_trajectory.png}
%     \caption{Optimisation of the distance to the granular material desired position manipulating the rigid-body trajectory.}
%     \label{fig:optimisation}
% \end{figure}

